Hiring as Exploration

This paper views hiring as a contextual bandit problem: to find the best workers over time, firms must balance exploitation (selecting from groups with proven track records) with exploration (selecting from under-represented groups to learn about quality). Yet modern hiring algorithms, based on supervised learning approaches, are designed solely for exploitation. Instead, we build a resume screening algorithm that values exploration by evaluating candidates according to their statistical upside potential. Using data from professional services recruiting within a Fortune 500 firm, we show that this approach improves the quality (as measured by eventual hiring rates) of candidates selected for an interview, while also increasing demographic diversity, relative to the firm's existing practices. The same is not true for traditional supervised learning based algorithms, which improve hiring rates but select far fewer Black and Hispanic applicants. Together, our results highlight the importance of incorporating exploration in developing decision-making algorithms that are potentially both more efficient and equitable.

==> Output/Dec2022/summary_demographics.tex <==
\begin{tabular}{lcc} \toprule \toprule
Variable & Observations & Share of Previous Rd.\\
\addlinespace \hline \addlinespace

Black & & \\
\hspace{3mm} Applications &        7,715 & \\
\hspace{3mm} Interviewed &          217 & 0.028 \\
\hspace{3mm} Offered &           11 &11.000 \\
\hspace{3mm} Hired &            8 & 0.037 \\

Hispanic & & \\
\hspace{3mm} Applications &        3,694 & \\
\hspace{3mm} Interviewed &          210 & 0.057 \\
\hspace{3mm} Offered &           31 &31.000 \\
\hspace{3mm} Hired &           16 & 0.076 \\

Asian & & \\
\hspace{3mm} Applications &       51,532 & \\
\hspace{3mm} Interviewed &        2,766 & 0.054 \\
\hspace{3mm} Offered &          583 &583.000 \\
\hspace{3mm} Hired &          308 & 0.111 \\

White & & \\
\hspace{3mm} Applications &       25,762 & \\
\hspace{3mm} Interviewed &        1,561 & 0.061 \\
\hspace{3mm} Offered &          362 &362.000 \\
\hspace{3mm} Hired &          190 & 0.122 \\

Female & & \\
\hspace{3mm} Applications &       29,425 & \\
\hspace{3mm} Interviewed &        1,541 & 0.052 \\
\hspace{3mm} Offered &          306 &306.000 \\
\hspace{3mm} Hired &          181 & 0.117 \\

Male & & \\
\hspace{3mm} Applications &       59,278 & \\
\hspace{3mm} Interviewed &        3,213 & 0.054 \\
\hspace{3mm} Offered &          681 &681.000 \\
\hspace{3mm} Hired &          341 & 0.106 \\

Interviewed & & \\
\hspace{3mm} Applications &        4,754 & \\
\hspace{3mm} Interviewed &        4,754 & 1.000 \\
\hspace{3mm} Offered &          987 &987.000 \\
\hspace{3mm} Hired &          522 & 0.110 \\

Hired & & \\
\hspace{3mm} Applications &          522 & \\
\hspace{3mm} Interviewed &          522 & 1.000 \\
\hspace{3mm} Offered &          522 &522.000 \\
\hspace{3mm} Hired &          522 & 1.000 \\
\addlinespace \bottomrule \bottomrule
\end{tabular}


==> Output/Dec2022/summary_jobfam.tex <==
\begin{tabular}{lcc} \toprule \toprule
Variable & Observations & Share of Previous Rd. \\
\addlinespace \hline \addlinespace

All Job Families & & \\
\hspace{3mm} Applications &       88,703 & \\
\hspace{3mm} Interviewed &        4,754 &  0.054 \\
\hspace{3mm} Offered &          987 & 987.000 \\
\hspace{3mm} Hired &          522 &  0.110 \\

Business Analysts & & \\
\hspace{3mm} Applications &       44,146 & \\
\hspace{3mm} Interviewed &        3,605 &  0.082 \\
\hspace{3mm} Offered &          565 & 565.000 \\
\hspace{3mm} Hired &          317 &  0.088 \\

Data Scientists & & \\
\hspace{3mm} Applications &       44,557 & \\
\hspace{3mm} Interviewed &        1,149 &  0.026 \\
\hspace{3mm} Offered &          422 & 422.000 \\
\hspace{3mm} Hired &          205 &  0.178 \\
\addlinespace \bottomrule \bottomrule
\end{tabular}


==> Output/Jan2021/summary.tex <==
\begin{tabular}{lccc} \toprule \toprule
Variable            &       Mean Training   & Mean Test & Mean Overall \\
\addlinespace \hline \addlinespace
Black &   0.09 &   0.09 &   0.09 \\
Hispanic &   0.04 &   0.04 &   0.04 \\
Asian &   0.57 &   0.59 &   0.58 \\
White &   0.30 &   0.28 &   0.29 \\
Male &   0.68 &   0.66 &   0.67 \\
Female &   0.32 &   0.34 &   0.33 \\
Referred &   0.14 &   0.11 &   0.13 \\
B.A. Degree &   0.23 &   0.24 &   0.24 \\
Associate Degree &   0.01 &   0.01 &   0.01 \\
Master's Degree &   0.61 &   0.64 &   0.63 \\
Ph.D. &   0.07 &   0.07 &   0.07 \\
Attended a U.S. College &   0.75 &   0.80 &   0.77 \\
Attended Elite U.S. College &   0.13 &   0.14 &   0.13 \\
Interviewed &   0.05 &   0.05 &   0.05 \\
Hired &   0.01 &   0.01 &   0.01 \\
Observations &       48,719 &       39,947 &       88,666 \\
\addlinespace \bottomrule \bottomrule
\end{tabular}


==> Output/RefereeRequestsMay2024/bonus_analysis_byrace_candidate_baplus_with_controls.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{4}{c}}
\hline\hline
                         &\multicolumn{1}{c}{Bonus}&\multicolumn{1}{c}{Blinded Bonus}&\multicolumn{1}{c}{UCB Score}&\multicolumn{1}{c}{UCB Blinded Score}\\
                         &\multicolumn{1}{c}{(1)}   &\multicolumn{1}{c}{(2)}   &\multicolumn{1}{c}{(3)}   &\multicolumn{1}{c}{(4)}   \\
\hline
Graduate Education=1     &     -0.0158***&     -0.0162***&     -0.0512***&     -0.0388***\\
                         &  (0.000990)   &  (0.000954)   &   (0.00187)   &   (0.00176)   \\
[1em]
Graduate Education=1 $\times$ Asian&     -0.0264***&     -0.0180***&     -0.0143***&     -0.0355***\\
                         &   (0.00133)   &   (0.00129)   &   (0.00252)   &   (0.00237)   \\
[1em]
Graduate Education=1 $\times$ Black/Hispanic&      -0.101***&     0.00346** &      -0.171***&   0.0000607   \\
                         &   (0.00170)   &   (0.00164)   &   (0.00321)   &   (0.00302)   \\
\hline
Observations             &       35526   &       35526   &       35526   &       35526   \\
\hline\hline
\end{tabular}
}


==> Output/RefereeRequestsMay2024/bonusdiff_analysis_candidate_baplus.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{2}{c}}
\hline\hline
                         &\multicolumn{1}{c}{Bonus Difference}&\multicolumn{1}{c}{Bonus Difference}\\
                         &\multicolumn{1}{c}{(1)}   &\multicolumn{1}{c}{(2)}   \\
\hline
Graduate Education=1     &     0.00213** &      0.0428***\\
                         &  (0.000894)   &  (0.000712)   \\
[1em]
Graduate Education=1 $\times$ Asian&     0.00731***&               \\
                         &   (0.00121)   &               \\
[1em]
Graduate Education=1 $\times$ Black/Hispanic&       0.105***&               \\
                         &   (0.00157)   &               \\
[1em]
Graduate Education=1 $\times$ Female=1&               &     -0.0237***\\
                         &               &   (0.00123)   \\
\hline
Observations             &       35542   &       39087   \\
\hline\hline
\end{tabular}
}


==> Output/RefereeRequestsMay2024/bonusdiff_analysis_racegender_table.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{2}{c}}
\hline\hline
                         &\multicolumn{1}{c}{Bonus Difference}&\multicolumn{1}{c}{Bonus Differences}\\
                         &\multicolumn{1}{c}{(1)}   &\multicolumn{1}{c}{(2)}   \\
\hline
Asian                    &      0.0301***&               \\
                         &  (0.000619)   &               \\
                         &               &               \\
[1em]
Black/Hispanic           &     -0.0315***&               \\
                         &  (0.000853)   &               \\
[1em]
Female                 &               &    -0.00677***\\
                         &               &  (0.000586)   \\
\hline
Observations             &       35542   &       39087   \\
\hline\hline
\end{tabular}
}


==> Output/RefereeRequestsMay2024/mistake_score_ratios.tex <==
% matrix: ratios file: Output/RefereeRequestsMay2024/mistake_score_ratios.tex  28 May 2024 20:03:36
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{|l|l|l|l|l|}\hline  
 & Correlation  & Humans  & SL  & UCB  \\ \hline  
Elite &      0.13 &      0.93 &      1.19 &      1.13 \\  
Referral &      0.19 &      0.94 &      1.19 &      1.26 \\  
International &      0.03 &      0.96 &      1.40 &      1.40 \\  
PhD &     0.03 &      1.1 &      1.17 &      1.19 \\ \hline 
\end{tabular}
}


==> Output/RefereeRequestsMay2024/mistakes_covars_balance.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{3}{c}}
\hline\hline
                    &\multicolumn{1}{c}{High Human, Low SL Scores}&\multicolumn{1}{c}{Low Human, High SL Score}&\multicolumn{1}{c}{Difference (1)-(2)}\\
\hline
Master's Degree     &       0.74 &       0.50 &        0.24***\\
                    &     (0.44) &     (0.50) &      (0.01)   \\
International Applicant&       0.39 &       0.33 &        0.05***\\
                    &     (0.49) &     (0.47) &      (0.01)   \\
Attended International Elite College&       0.08 &       0.08 &       -0.00   \\
                    &     (0.27) &     (0.28) &      (0.00)   \\
Attended Elite U.S. College&       0.22 &       0.05 &        0.17***\\
                    &     (0.41) &     (0.22) &      (0.01)   \\
Attended Top 50 U.S. College&       0.33 &       0.17 &        0.16***\\
                    &     (0.47) &     (0.37) &      (0.01)   \\
   \\  \textbf{Work History} \vspace{.5em}&            &            &               \\
Referred            &       0.17 &       0.03 &        0.14***\\
                    &     (0.37) &     (0.16) &      (0.00)   \\
Nontraditional Educational Background&       0.02 &       0.07 &       -0.05***\\
                    &     (0.13) &     (0.25) &      (0.00)   \\
Has a Quantitative Background&       0.27 &       0.22 &        0.04***\\
                    &     (0.44) &     (0.42) &      (0.01)   \\
   \\  \textbf{Demographics} \vspace{.5em}&            &            &               \\
Female Applicant    &       0.28 &       0.39 &       -0.11***\\
                    &     (0.45) &     (0.49) &      (0.01)   \\
Black/Hispanic Applicant&       0.12 &       0.14 &       -0.02***\\
                    &     (0.32) &     (0.34) &      (0.01)   \\
Asian Applicant     &       0.57 &       0.48 &        0.08***\\
                    &     (0.50) &     (0.50) &      (0.01)   \\
 
  \\  \textbf{Outcomes} \vspace{.5em} &            &            &               \\
Offered             &       0.13 &       0.28 &       -0.15***\\
                    &     (0.34) &     (0.45) &      (0.04)   \\
Hired               &       0.07 &       0.17 &       -0.11***\\
                    &     (0.25) &     (0.38) &      (0.03)   \\
\hline\hline
\end{tabular}
}


==> Output/RefereeRequestsMay2024/mistakes_mean_model_scores.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{3}{c}}
\hline\hline
                    &\multicolumn{1}{c}{Not Hired if Interviewed}&\multicolumn{1}{c}{Hired if Interviewed}&\multicolumn{1}{c}{Difference (1)-(2)}\\
\hline
 \\  \emph{Candidate Elite=1} \vspace{.5em}&            &            &               \\
sH                  &       0.60 &       0.56 &        0.04   \\
                    &     (0.21) &     (0.14) &      (0.03)   \\
updating\_SL         &       0.43 &       0.55 &       -0.11*  \\
                    &     (0.22) &     (0.27) &      (0.06)   \\
logUCB              &       0.24 &       0.28 &       -0.04   \\
                    &     (0.16) &     (0.16) &      (0.04)   \\
 \\  \emph{Candidate Elite=0} \vspace{.5em}&            &            &               \\
sH                  &       0.58 &       0.55 &        0.03*  \\
                    &     (0.20) &     (0.20) &      (0.01)   \\
updating\_SL         &       0.39 &       0.49 &       -0.10***\\
                    &     (0.21) &     (0.22) &      (0.02)   \\
logUCB              &       0.26 &       0.33 &       -0.07***\\
                    &     (0.15) &     (0.18) &      (0.01)   \\
 \\  \emph{Candidate Int=1} \vspace{.5em}&            &            &               \\
sH                  &       0.59 &       0.57 &        0.02   \\
                    &     (0.22) &     (0.17) &      (0.02)   \\
updating\_SL         &       0.38 &       0.53 &       -0.15***\\
                    &     (0.22) &     (0.24) &      (0.03)   \\
logUCB              &       0.24 &       0.34 &       -0.10***\\
                    &     (0.16) &     (0.18) &      (0.02)   \\
 \\  \emph{Candidate Int=0} \vspace{.5em}&            &            &               \\
sH                  &       0.58 &       0.55 &        0.03*  \\
                    &     (0.19) &     (0.21) &      (0.02)   \\
updating\_SL         &       0.41 &       0.48 &       -0.08***\\
                    &     (0.20) &     (0.22) &      (0.02)   \\
logUCB              &       0.27 &       0.32 &       -0.05***\\
                    &     (0.15) &     (0.17) &      (0.01)   \\
 \\  \emph{Candidate Ref=1} \vspace{.5em}&            &            &               \\
sH                  &       0.75 &       0.70 &        0.05***\\
                    &     (0.15) &     (0.14) &      (0.02)   \\
updating\_SL         &       0.45 &       0.54 &       -0.09***\\
                    &     (0.21) &     (0.23) &      (0.03)   \\
logUCB              &       0.28 &       0.35 &       -0.07***\\
                    &     (0.16) &     (0.19) &      (0.02) \\
\\  \emph{Candidate\_Ref=0} \vspace{.5em}&            &            &               \\
sH                  &       0.53 &       0.48 &        0.05***\\
                    &     (0.19) &     (0.18) &      (0.02)   \\
updating\_SL         &       0.38 &       0.48 &       -0.10***\\
                    &     (0.20) &     (0.23) &      (0.02)   \\
logUCB              &       0.25 &       0.31 &       -0.06***\\
                    &     (0.15) &     (0.17) &      (0.01)   \\
\hline\hline
\end{tabular}
}


==> Output/features.tex <==
\begin{tabular}{lccc} \toprule \toprule
Variable            &       Mean Training   & Mean Test & Mean Overall \\
\addlinespace \hline \addlinespace
Worked at a Fortune 500 Co. &   0.02 &   0.02 &   0.02 \\
Has a Quantitative Background &   0.23 &   0.27 &   0.25 \\
Attended School in China & 0.07 & 0.08 & 0.08 \\
Attended School in Europe & 0.05 & 0.05 & 0.05 \\
Attended School in India & 0.21 & 0.24 & 0.22\\
Attended School in Latin America & 0.01 & 0.01 & 0.01 \\
Attended School in Middle East/Africa & 0.01 & 0.02 & 0.02\\
Attended School in Other Asian Country & 0.02 & 0.02 & 0.02\\
Attended Elite International School & 0.09 & 0.10 & 0.10\\
Attended US News Top 25 Ranked College & 0.14 & 0.14 & 0.14 \\
Attended US News Top 50 Ranked College & 0.27 & 0.28 & 0.28 \\
Military Experience & 0.04  & 0.04 & 0.04 \\
Number of Applications & 3.5  & 3.8 & 3.5 \\
Number of Unique Degrees & 1.7  & 1.75 & 1.7\\
Number of Work Histories & 3.8  & 4.0 & 3.9 \\
Has Service Sector Experience & 0.01  & 0.01  & 0.01 \\
Major Description Business Management & 0.17 & 0.15 & 0.17 \\
Major Description Computer Science & 0.14 & 0.13 & 0.14\\
Major Description Finance/Economics & 0.14 & 0.13 & 0.14\\
Major Description Engineering & 0.06 & 0.06 & 0.06 \\
Major Description None & 0.20 & 0.25 & 0.22\\
Observations &       48,719 &       39,947 &       88,666 \\
\addlinespace \bottomrule \bottomrule
\end{tabular}

==> preambles/header_beamer.tex <==
% Typesetting
	\usepackage{amsfonts}
	\usepackage{amssymb}
	\usepackage{amsmath}

	\usepackage{subfig}

	\usepackage{graphicx}
    
    \usepackage{multicol}
    \usepackage{tikz}
    \usetikzlibrary{calc,intersections}
    
    \usepackage{dcolumn}
    
    \usepackage{accents}
    \usepackage{adjustbox}

% Bibliography
    % \usepackage[style=authoryear-comp,natbib=true,backend=biber]{biblatex}
    % \addbibresource{Bibliography.bib}
    % \usepackage{csquotes}
	\usepackage{natbib}
 	%\bibliographystyle{apalike}
 	\bibliographystyle{aer}
	
	\usepackage{bibunits}
	\defaultbibliography{Bibliography.bib}  
	%\defaultbibliographystyle{apalike}
	\defaultbibliographystyle{aer}

	
% Links
	\usepackage{hyperref}
	\hypersetup{
    colorlinks=true,
    linkcolor=black,
    filecolor=magenta,      
    urlcolor=blue,
    citecolor = black
}
	\usepackage{cleveref}

% Todonotes
	\usepackage[framemethod=tikz]{mdframed}
	\usepackage{todonotes}
	\presetkeys{todonotes}{color=black!5,inline}{} % noline

% Boxes
    \usepackage{tcolorbox}
    \newtcbox{\feedback}{nobeforeafter,colframe=black,colback=white,boxrule=0.5pt,arc=2pt,
      boxsep=0pt,left=2pt,right=2pt,top=2pt,bottom=2pt,tcbox raise base}
      
% Theorems
    \usepackage{amsthm}
     
    \newtheorem{thm}{Theorem}
    \newtheorem{asm}{Assumption}
    \newtheorem{con}{Conjecture}
    \newtheorem{prop}{Proposition}
    \newtheorem{lem}{Lemma}
    \newtheorem{cor}{Corollary}
    \newtheorem{rem}{Remark}
    \newtheorem{defn}{Definition}

%Packages and commands for column widths in tables
\usepackage{array}
\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash}m{#1}}
\newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{R}[1]{>{\raggedleft\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}

%Turn off toolbar
\setbeamertemplate{navigation symbols}[default]
\beamertemplatenavigationsymbolsempty  


%Macro for wrapping text in underbrace
\usepackage{ragged2e}
\newlength\ubwidth
\newcommand\wrapunderbrace[2]{\settowidth\ubwidth{$#1$}\underbrace{#1}_{\parbox{\ubwidth}{\scriptsize\RaggedRight#2}}}


%This makes citations smaller
\makeatletter
\DeclareRobustCommand\citep
{\begingroup\footnotesize\NAT@swatrue\let\NAT@ctype\z@\NAT@partrue
    \@ifstar{\NAT@fulltrue\NAT@citetp}{\NAT@fullfalse\NAT@citetp}}
\makeatother

==> preambles/header_old.tex <==
\usepackage{amsmath,amsthm,amssymb,amsfonts,mathrsfs}
\usepackage{fullpage}
\usepackage{microtype} % makes pdf look better
\usepackage{graphicx,tabularx,color}
\usepackage[small,bf,up]{caption}
\usepackage{subfigure}
\usepackage{venndiagram}
\usepackage{subfiles}
\usepackage{setspace,booktabs}
\usepackage[flushleft]{threeparttable}
\usepackage{pdflscape,comment,soul}
%\usepackage{pdfsync}
\usepackage{multirow,rotating,bigints}
\usepackage[ruled,vlined]{algorithm2e}
\usepackage{float,epsfig,tabularx}
\usepackage{epstopdf}
\usepackage{indentfirst}
\usepackage{rotating}
\usepackage{type1cm}
\usepackage[utf8x]{inputenc}
%\usepackage[T1]{fontenc}
\usepackage{natbib}

\usepackage{array}
\usepackage{tikz,pgfplots}
\usepackage{pgfplotstable,filecontents}
\usepackage[colorlinks]{hyperref}
\usepackage[12pt]{moresize}
\usepackage{longtable}
\usepackage{xr}
\usepackage{dcolumn}
\usetikzlibrary{positioning,shapes,backgrounds}
\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{R}[1]{>{\raggedleft\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}

    \newlength\fheight
    \newlength\fwidth

    %\externaldocument{OnlineAppendix_v2017_0824}

%declare argmax
\DeclareMathOperator*{\argmax}{argmax} % thin space, limits underneath in displays

%\usepackage{showkeys}
\renewcommand{\cite}{\citep}
\newcommand{\cn}{\citet}
\newcommand{\cy}{\citeyear}
\newcommand{\ca}{\citeauthor}
%\doublespacing
\newcommand{\PSbox}[3]{\mbox{\rule{0in}{#3}\special{psfile=#1}\hspace{#2}}}
\def\E{{\rm E}}
\def\e{\varepsilon}
\def\sdf{\Lambda}
\def\w{\textsc{w}}
\def\eea{\end{eqnarray*}}
\def\bea{\begin{eqnarray*}}
\renewcommand{\[}{\begin{equation}}
\renewcommand{\]}{\end{equation}}
\newcommand{\bi}{\begin{itemize}}
\newcommand{\ei}{\end{itemize}}


\newtheorem{theorem}{Theorem}
\renewcommand{\qed}{\ \rule{0.5em}{0.5em}}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}{Lemma}
\newtheorem{definition}{Definition}
\newtheorem{example}{Example}
\newtheorem{corrolary}{Corrolary}
\renewenvironment{proof}[1][Proof]{\textbf{#1.} }{\ \rule{0.5em}{0.5em}}

%This command changes the appearance of the \subsubsection header
%\makeatletter
%\renewcommand{\subsubsection}{\vspace*{-0pt}\@startsection{subsubsection}{3}{\z@}{-\baselineskip}{0.01\baselineskip}
%{\normalfont \normalsize\bfseries}}
%\makeatother

%\renewcommand{\thesection}{\Alph{section}}
\renewcommand{\thesection}{\arabic{section}}
\renewcommand{\thesubsection}{\thesection.\arabic{subsection}}
\renewcommand{\thesubsubsection}{\thesubsection.\arabic{subsubsection}}
\renewcommand{\figurename}{\footnotesize\bf Figure}
\renewcommand{\tablename}{\bf Table}

\newcommand{\PB}[1]{{\color{red}{[PB: #1]}}}
\newcommand{\DL}[1]{{\color{blue}{[DL: #1]}}}
\newcommand{\LR}[1]{{\color{purple}{[LR: #1]}}}

%\renewcommand{\ignore}[1]{ }




\setcounter{tocdepth}{3}
\setcounter{secnumdepth}{3}

%\setlength{\textwidth}{6.5in} \setlength{\oddsidemargin}{0.0in} \setlength{\textheight}{9.65in}
%\setlength{\topmargin}{-0.1in} \setlength{\headheight}{0.0in} \footnotesep 9pt
%\setlength{\baselineskip}{.75\baselineskip}

\clubpenalty = 10000
\widowpenalty = 10000


\setlength{\parskip}{0.2mm}

\usepackage{pgfplotstable}
\pgfplotsset{compat=1.18}

%\usetikzlibrary{external}
%\tikzexternalize[prefix=tikz/,shell escape=-enable-write18]
%\newcommand{\plotref}[1]{\tikzexternaldisable\ref{#1}\tikzexternalenable}

%\usetikzlibrary{external}
%\tikzexternalize[prefix=tikz/,shell escape=-enable-write18]
%\newcommand{\plotref}[1]{\tikzexternaldisable\ref{#1}\tikzexternalenable}
\usepackage{geometry}
\geometry{left=1in}
\geometry{right=1 in}
\geometry{top=.9in}
\geometry{bottom=.9in}
\linespread{1.33}


\usepackage{caption}
\captionsetup{labelformat=empty,labelsep=none}


